Learning Generative Models of Structured Signals from Their Superposition Using GANs with Application to Denoising and Demixing

Recently, Generative Adversarial Networks (GANs) have emerged as a popular alternative for modeling complex high dimensional distributions. Most of the existing works implicitly assume that the clean samples from the target distribution are easily available. However, in many applications, this assumption is violated. In this paper, we consider the observation setting when the samples from target distribution are given by the superposition of two structured components and leverage GANs for learning the structure of the components. We propose two novel frameworks: denoising-GAN and demixing-GAN. The denoising-GAN assumes access to clean samples from the second component and try to learn the other distribution, whereas demixing-GAN learns the distribution of the components at the same time. Through extensive numerical experiments, we demonstrate that proposed frameworks can generate clean samples from unknown distributions, and provide competitive performance in tasks such as denoising, demixing, and compressive sensing.

==> All_talks/latexdefs.tex <==
\newcommand{\redbold}[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\OPT}{\ensuremath{\mathit{OPT}}}
\newcommand{\EMD}{\ensuremath{\textnormal{EMD}}}
\newcommand{\sEMD}{\ensuremath{\textnormal{sEMD}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Mmodel}{\ensuremath{\mathcal{M}}}
\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\Msupports}{\ensuremath{\mathbb{M}}}
\newcommand{\Params}{\ensuremath{\mathcal{P}}}
\newcommand{\supp}{\ensuremath{\textnormal{supp}}}
\newcommand{\rank}{\ensuremath{\textnormal{rank}}}
\newcommand{\poly}{\ensuremath{\textnormal{poly}}}
\newcommand{\diag}{\ensuremath{\textnormal{diag}}}
\newcommand{\betahat}{\ensuremath{\widehat{\beta}}}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\parens}{\lparen}{\rparen}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\Green}[1]{\textcolor{Green}{#1}}
%\newcommand{\cit}[1]{\textcolor{blue!60}{#1}}
\newcommand{\cit}[1]{\footnotesize{\textcolor{gray}{#1}}}

\DeclareMathOperator{\Mcol}{col}
\DeclareMathOperator{\Mrow}{row}
\DeclareMathOperator{\Mnull}{null}

% Swap the definition of the starred version of the delimiters, so that the
% non-starred versions automatically resize.
\makeatletter
\let\oldparens\parens
\def\parens{\@ifstar{\oldparens}{\oldparens*}}
%
\let\oldnorm\norm
\def\norm{\@ifstar{\oldnorm}{\oldnorm*}}
%
\let\oldceil\ceil
\def\ceil{\@ifstar{\oldceil}{\oldceil*}}
%
\let\oldfloor\floor
\def\floor{\@ifstar{\oldfloor}{\oldfloor*}}
%
\let\oldabs\abs
\def\abs{\@ifstar{\oldabs}{\oldabs*}}
\makeatother

% for indented lines in algorithmicx
\begin{comment}
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
\setlength\@tempdima{\algorithmicindent}%
\OldStatex\hskip\dimexpr#1\@tempdima\relax}
\makeatother
\end{comment}

%sqrt
\makeatletter
\let\oldr@@t\r@@t
\def\r@@t#1#2{%
\setbox0=\hbox{$\oldr@@t#1{#2\,}$}\dimen0=\ht0
\advance\dimen0-0.2\ht0
\setbox2=\hbox{\vrule height\ht0 depth -\dimen0}%
{\box0\lower0.4pt\box2}}
\LetLtxMacro{\oldsqrt}{\sqrt}
\renewcommand*{\sqrt}[2][\ ]{\oldsqrt[#1]{#2}}
\makeatother

\def\x{{\mathbf x}}
\def\R{{\mathbb{R}}}
\def\E{{\mathbb{E}}}
\def\L{{\cal L}}
\def\lin{\text{lin}}
%\newcommand{\norm}[1]{\|#1\|}
\def\rank{\text{rank}}
\def\O{{\mathcal{O}}}
\def\D{{\mathcal{D}}}
\def\X{\mathcal{X}}
\def\N{\mathcal{N}}
\def\P{{\mathcal{P}}}
\def\pr{\mathbb{P}}
\def\la{\lambda}
\def\si{\sigma}
\def\A{\mathcal{A}}
\def\T{\widetilde}
\def\Ta{{\mathcal{T}}}
\def\H{{\mathcal{H}}}
\def\M{\mathcal{M}}
\def\U{\mathbb{U}}
\def\n{\Big{\|}}
\def\bS{\bar{S}}
\def\'{\prime}
\def\Otilde{{\widetilde{O}}}
\def\C{\mathcal{C}}
\def\poly{\text{poly}}
  

